Active Learning with Expected Error Reduction

Active learning has been studied extensively as a method for efficient data collection. Among the many approaches in literature, Expected Error Reduction (EER) (Roy and McCallum) has been shown to be an effective method for active learning: select the candidate sample that, in expectation, maximally decreases the error on an unlabeled set. However, EER requires the model to be retrained for every candidate sample and thus has not been widely used for modern deep neural networks due to this large computational cost. In this paper we reformulate EER under the lens of Bayesian active learning and derive a computationally efficient version that can use any Bayesian parameter sampling method (such as arXiv:1506.02142). We then compare the empirical performance of our method using Monte Carlo dropout for parameter sampling against state of the art methods in the deep active learning literature. Experiments are performed on four standard benchmark datasets and three WILDS datasets (arXiv:2012.07421). The results indicate that our method outperforms all other methods except one in the data shift scenario: a model dependent, non-information theoretic method that requires an order of magnitude higher computational cost (arXiv:1906.03671).

==> tables/aucs.tex <==
% \toprule
\begin{table*}[ht]
\centering
\small
\begin{tabular}{ | l | cccccccc |}
\hline Dataset & BADGE & Coreset\_Greedy & MEZL & Entropy & Entropy\_MC & Random & MELL & BALD \\ \hline\hline
\multirow{2}{*}{cifar10\_covshift} &  \textbf{84.28} &  \textbf{84.19} & 83.75 &  \textbf{84.34} & 84.13 & 83.10 & 84.11 & 84.09 \\
 &  \textbf{$\pm$ 0.09} &  \textbf{$\pm$ 0.09} & $\pm$ 0.12 &  \textbf{$\pm$ 0.08} & $\pm$ 0.09 & $\pm$ 0.11 & $\pm$ 0.09 & $\pm$ 0.08  \\ \hline 
 \multirow{2}{*}{cifar10\_noshift} &  \textbf{81.68} &  \textbf{81.58} & 81.25 &  \textbf{81.66} &  \textbf{81.65} & 80.65 &  \textbf{81.74} &  \textbf{81.63} \\
 &  \textbf{$\pm$ 0.21} &  \textbf{$\pm$ 0.12} & $\pm$ 0.30 &  \textbf{$\pm$ 0.12} &  \textbf{$\pm$ 0.10} & $\pm$ 0.12 &  \textbf{$\pm$ 0.10} &  \textbf{$\pm$ 0.10}  \\ \hline 
 \multirow{2}{*}{cifar100\_covshift} & 48.12 & 48.19 &  \textbf{48.46} & 47.35 & 47.93 & 48.16 &  \textbf{48.51} &  \textbf{48.46} \\
 & $\pm$ 0.16 & $\pm$ 0.12 &  \textbf{$\pm$ 0.11} & $\pm$ 0.13 & $\pm$ 0.15 & $\pm$ 0.13 &  \textbf{$\pm$ 0.12} &  \textbf{$\pm$ 0.18}  \\ \hline 
 \multirow{2}{*}{cifar100\_noshift} &  &  \textbf{44.30} & 43.82 & 42.68 & 42.83 & 43.83 & 43.96 & 43.94 \\
 &  &  \textbf{$\pm$ 0.09} & $\pm$ 0.11 & $\pm$ 0.11 & $\pm$ 0.11 & $\pm$ 0.09 & $\pm$ 0.09 & $\pm$ 0.11  \\ \hline 
 \multirow{2}{*}{svhn\_covshift} &  \textbf{91.26} & 90.84 & 90.76 &  \textbf{91.28} &  \textbf{91.10} & 89.52 & 91.09 &  \textbf{91.09} \\
 &  \textbf{$\pm$ 0.08} & $\pm$ 0.09 & $\pm$ 0.12 &  \textbf{$\pm$ 0.10} &  \textbf{$\pm$ 0.09} & $\pm$ 0.10 & $\pm$ 0.08 &  \textbf{$\pm$ 0.09}  \\ \hline 
 \multirow{2}{*}{svhn\_noshift} &  \textbf{91.80} &  \textbf{91.71} & 91.48 &  \textbf{91.80} &  \textbf{91.80} & 90.41 &  \textbf{91.73} &  \textbf{91.75} \\
 &  \textbf{$\pm$ 0.05} &  \textbf{$\pm$ 0.05} & $\pm$ 0.05 &  \textbf{$\pm$ 0.05} &  \textbf{$\pm$ 0.05} & $\pm$ 0.04 &  \textbf{$\pm$ 0.05} &  \textbf{$\pm$ 0.04}  \\ \hline 
 \multirow{2}{*}{iwildcam\_shift} &  & 83.37 &  \textbf{85.22} & 76.54 & 78.92 & 79.84 &  \textbf{85.17} & 80.14 \\
 &  & $\pm$ 0.16 &  \textbf{$\pm$ 0.12} & $\pm$ 0.37 & $\pm$ 0.13 & $\pm$ 0.11 &  \textbf{$\pm$ 0.11} & $\pm$ 0.11  \\ \hline 
 \multirow{2}{*}{iwildcam\_noshift} &  &  \textbf{92.40} & 92.24 & 91.57 & 91.64 & 88.03 &  \textbf{92.47} & 91.84 \\
 &  &  \textbf{$\pm$ 0.07} & $\pm$ 0.05 & $\pm$ 0.06 & $\pm$ 0.05 & $\pm$ 0.08 &  \textbf{$\pm$ 0.07} & $\pm$ 0.07  \\ \hline 
 \multirow{2}{*}{camelyon\_shift} &  \textbf{97.67} & 92.20 & 96.63 &  \textbf{97.62} & 96.15 & 96.59 & 96.59 & 95.79 \\
 &  \textbf{$\pm$ 0.06} & $\pm$ 0.18 & $\pm$ 0.02 &  \textbf{$\pm$ 0.03} & $\pm$ 0.18 & $\pm$ 0.04 & $\pm$ 0.20 & $\pm$ 0.42  \\ \hline 
 \multirow{2}{*}{camelyon\_noshift} &  \textbf{98.12} & 97.28 & 97.06 &  \textbf{98.13} &  \textbf{98.11} & 97.02 & 98.02 &  \textbf{98.12} \\
 &  \textbf{$\pm$ 0.04} & $\pm$ 0.03 & $\pm$ 0.06 &  \textbf{$\pm$ 0.03} &  \textbf{$\pm$ 0.04} & $\pm$ 0.03 & $\pm$ 0.03 &  \textbf{$\pm$ 0.03}  \\ \hline 
 \multirow{2}{*}{fmow\_shift} &  &  \textbf{33.22} &  \textbf{33.17} & 31.84 & 32.12 & 32.33 &  \textbf{33.08} &  \textbf{33.17} \\
 &  &  \textbf{$\pm$ 0.10} &  \textbf{$\pm$ 0.12} & $\pm$ 0.11 & $\pm$ 0.10 & $\pm$ 0.13 &  \textbf{$\pm$ 0.09} &  \textbf{$\pm$ 0.09}  \\ \hline 
 \multirow{2}{*}{fmow\_noshift} &  &  \textbf{36.67} & 36.43 & 34.75 & 34.90 & 35.10 &  \textbf{36.43} &  \textbf{36.48} \\
 &  &  \textbf{$\pm$ 0.11} & $\pm$ 0.12 & $\pm$ 0.13 & $\pm$ 0.15 & $\pm$ 0.11 &  \textbf{$\pm$ 0.15} &  \textbf{$\pm$ 0.15}  \\ \hline 
 \multirow{2}{*}{mnist\_noshift} &  \textbf{97.60} & 97.35 & 96.71 & 97.28 & 97.27 & 96.23 &  \textbf{97.50} & 97.10 \\
 &  \textbf{$\pm$ 0.06} & $\pm$ 0.06 & $\pm$ 0.09 & $\pm$ 0.06 & $\pm$ 0.07 & $\pm$ 0.09 &  \textbf{$\pm$ 0.04} & $\pm$ 0.06  \\ \hline 
 \multirow{2}{*}{mnist\_covshift} &  &  \textbf{99.51} & 99.33 &  \textbf{99.51} & 99.48 & 99.30 & 99.45 & 99.45 \\
 &  &  \textbf{$\pm$ 0.02} & $\pm$ 0.02 &  \textbf{$\pm$ 0.02} & $\pm$ 0.01 & $\pm$ 0.02 & $\pm$ 0.01 & $\pm$ 0.01  \\ \hline 
 \multirow{2}{*}{mnist-fashion\_noshift} &  &  \textbf{93.18} & 90.86 &  \textbf{93.34} & 92.31 & 89.83 & 91.81 & 91.96 \\
 &  &  \textbf{$\pm$ 0.13} & $\pm$ 0.44 &  \textbf{$\pm$ 0.17} & $\pm$ 0.31 & $\pm$ 0.43 & $\pm$ 0.33 & $\pm$ 0.25  \\ \hline 
 \multirow{2}{*}{mnist-fashion\_covshift} &  & 91.47 & 88.97 &  \textbf{91.88} & 90.87 & 89.12 & 90.09 & 89.97 \\
 &  & $\pm$ 0.14 & $\pm$ 0.57 &  \textbf{$\pm$ 0.07} & $\pm$ 0.38 & $\pm$ 0.57 & $\pm$ 0.35 & $\pm$ 0.38  \\ \hline
\end{tabular}
\caption{\label{tab:dataset-table} Area under the curve (AUC) of active learning curves for each method on each dataset. Cells contain mean AUC and standard deviation across 10 trials.}
\end{table*}

==> tables/macros.tex <==


\usepackage{amsfonts} 
\usepackage{amsmath}
%\usepackage{todonotes} % for comments
\usepackage{multirow}
%\newcommand{\steve}[1]{\todo[inline,color=green!20!white]{\textbf{Steve:} #1}}
\newcommand{\steve}[1]{{\color{red} Steve: #1}}
\newcommand{\daniel}[1]{{\color{orange} Daniel: #1}}
\newcommand{\julia}[1]{{\color{blue} Julia: #1}}
\newcommand{\moises}[1]{{\color{green} Moises: #1}}
\newcommand{\ehsan}[1]{{\color{magenta} Ehsan: #1}}

==> tables/saturation-shift.tex <==
% \toprule
\begin{table}[H]
\label{tab:saturation-shift-table}
\centering
\small
\begin{tabular}{|l||*{7}{c|}}\hline
\backslashbox{Method}{Dataset (shift)}
&\makebox[4em]{CIFAR10}&\makebox[4em]{CIFAR100}&\makebox[4em]{SVHN}
&\makebox[4em]{MNIST}&\makebox[4em]{iWildCam}&\makebox[4em]{Camelyon17}&\makebox[4em]{FMoW}\\\hline\hline
MELL       &\cellcolor{green!25}\textbf{35000}    &\cellcolor{green!25}\textbf{37000}    &\cellcolor{green!25}\textbf{26000}    &\cellcolor{green!25}\textbf{520} &\cellcolor{green!25}\textbf{35000*}   &36000             &\cellcolor{green!25}\textbf{37000*}\\\hline
MEZL       & 37000            &38000             &27000             &\cellcolor{green!25}\textbf{520}          &36000             &\textgreater40000 &38000\\\hline
BALD       &\cellcolor{green!25}\textbf{35000}    &38000    &27000             &680          &39000             &37000             &38000\\\hline
Entropy MC &36000             &38000             &\cellcolor{green!25}\textbf{26000}    &600 &40000             &38000             &\textgreater40000\\\hline
Entropy    &\cellcolor{green!25}\textbf{35000}    &38000             &\cellcolor{green!25}\textbf{26000}    &680 &\textgreater40000 &\cellcolor{green!25}\textbf{29000}   &\textgreater40000\\\hline
CoreSet    &36000          &39000            &27000           &\cellcolor{green!25}\textbf{520}            &36000 &\textgreater40000             &38000 \\\hline
BADGE      &\cellcolor{green!25}\textbf{35000}          &38000             &\cellcolor{green!25}\textbf{26000}         &-           &- &\cellcolor{green!25}\textbf{29000}             &- \\\hline
Random     &\textgreater40000 &39000             &36000             &\cellcolor{green!25}\textbf{520}          &\textgreater40000 &\textgreater40000 &40000\\\hline
\end{tabular}

% CIFAR10 0.9925
% CIFAR100 0.97
% SVHN 0.98
% MNIST 0.96
% iWildCam 0.98
% Camelyon17 0.995
% FMoW 0.95

\caption{ Saturation points on datasets with shift for each method. MELL is the best method on iWildCam and FMoW, and is on par with state of the art methods on all other datasets. Note that entropy outperforms all methods in Camelyon; an explanation for this is provided in \ref{sec:results}. Bold and green cell indicates that it is the best performing method, or on-par. Asterisk indicates sole best performing method.}
\end{table} 

% \backslashbox{Method}{Dataset (shift)}
% &\makebox[4em]{CIFAR10}&\makebox[4em]{CIFAR100}&\makebox[4em]{SVHN}
% &\makebox[4em]{MNIST}&\makebox[4em]{iWildCam}&\makebox[4em]{Camelyon17}&\makebox[4em]{FMoW}\\\hline\hline
% MELL       &\textbf{37000}    &\textbf{39000}    &\textbf{32000}    &\textbf{22000} &\textbf{38000*}   &36000             &\textbf{40000}\\\hline
% MEZL       &\textbf{37000}    &\textbf{40000}    &39000             &26000          &40000             &\textgreater40000 &\textbf{39000}\\\hline
% BALD       &\textbf{36000}    &\textbf{39000}    &\textbf{32000}    &\textbf{23000} &\textgreater40000 &37000             &\textbf{40000}\\\hline
% Entropy MC &\textbf{36000}    &\textbf{40000}    &\textbf{30000}    &\textbf{22000} &\textgreater40000 &38000             &\textgreater40000\\\hline
% Entropy    &\textbf{36000}    &\textbf{40000}    &\textbf{31000}    &\textbf{21000} &\textgreater40000 &\textbf{29000*}   &\textgreater40000\\\hline
% Random     &\textgreater40000 &\textgreater40000 &\textgreater40000 &27000          &\textgreater40000 &\textgreater40000 &\textgreater40000\\\hline
% \end{tabular}

==> tables/saturation.tex <==
% \toprule
\begin{table}[H]
\centering
\small

\begin{tabular}{|l||*{7}{c|}}\hline
\backslashbox{Method}{Dataset (no shift)}
&\makebox[4em]{CIFAR10}&\makebox[4em]{CIFAR100}&\makebox[4em]{SVHN}
&\makebox[4em]{MNIST}&\makebox[4em]{iWildCam}&\makebox[4em]{Camelyon17}&\makebox[4em]{FMoW}\\\hline\hline
MELL       &\cellcolor{green!25}\textbf{27500} &\cellcolor{green!25}\textbf{42500}    &\cellcolor{green!25}\textbf{22500} &\cellcolor{green!25}\textbf{440}              &\cellcolor{green!25}\textbf{22500}    &\cellcolor{green!25}\textbf{17500}    &\cellcolor{green!25}\textbf{27500}\\\hline
MEZL       &30000          &\cellcolor{green!25}\textbf{42500}    &27500          &520           &25000             &\textgreater55000 &\cellcolor{green!25}\textbf{27500}\\\hline
BALD       &\cellcolor{green!25}\textbf{27500} &\cellcolor{green!25}\textbf{42500}    &\cellcolor{green!25}\textbf{22500} &520                        &25000             &\cellcolor{green!25}\textbf{17500}    &\cellcolor{green!25}\textbf{27500}\\\hline
Entropy MC &\cellcolor{green!25}\textbf{27500} &\cellcolor{green!25}\textbf{42500}    &\cellcolor{green!25}\textbf{22500} &520                        &25000    &\cellcolor{green!25}\textbf{17500}    &30000\\\hline
Entropy    &\cellcolor{green!25}\textbf{27500} &\cellcolor{green!25}\textbf{42500}    &\cellcolor{green!25}\textbf{22500} &\cellcolor{green!25}\textbf{440}                        &25000    &\cellcolor{green!25}\textbf{17500}    &30000\\\hline
CoreSet    &30000          &42500            &\cellcolor{green!25}\textbf{22500}           &\cellcolor{green!25}\textbf{440}           &\cellcolor{green!25}\textbf{22500} &40000             &55000 \\\hline
BADGE      &\cellcolor{green!25}\textbf{27500}          &-             &\cellcolor{green!25}\textbf{22500}          &\cellcolor{green!25}\textbf{440}           &- &\textbf{17500}             &- \\\hline
Random     &37500          &45000             &47500          &680           &52500 &50000             &\textgreater55000\\\hline
\end{tabular}


% CIFAR10 0.98
% CIFAR100 0.98
% SVHN 0.9925
% MNIST 0.9800
% iWildCam 0.9800
% Camelyon17 0.9925
% FMoW 0.9800

\caption{\label{tab:saturation-no-shift-table} Saturation points on datasets with no shift for each method. MELL outperforms all other methods on MNIST, and is on-par with state of the art methods on all other datasets. Bold and green cell indicates that it is the best performing method, or on-par. Asterisk indicates sole best performing method.}
\end{table} 

% \backslashbox{Method}{Dataset (no shift)}
% &\makebox[4em]{CIFAR10}&\makebox[4em]{CIFAR100}&\makebox[4em]{SVHN}
% &\makebox[4em]{MNIST}&\makebox[4em]{iWildCam}&\makebox[4em]{Camelyon17}&\makebox[4em]{FMoW}\\\hline\hline
% MELL       &\textbf{37500} & \textbf{42500}   &\textbf{25000} &\textbf{440*} &\textbf{40000}    &\textbf{22500}    &\textbf{55000}\\\hline
% MEZL       &40000          &\textbf{45000}    &32500          &600           &47500             &\textgreater55000 &\textbf{55000}\\\hline
% BALD       &\textbf{35000} &\textbf{45000}    &\textbf{25000} &600           &\textbf{42500}    &\textbf{17500}    &\textbf{55000}\\\hline
% Entropy MC &\textbf{37500} &\textbf{45000}    &\textbf{22500} &520           &\textbf{40000}    &\textbf{20000}    &\textgreater55000\\\hline
% Entropy    &\textbf{35000} &\textbf{45000}    &\textbf{22500} &520           &\textbf{40000}    &\textbf{17500}    &\textgreater55000\\\hline
% Random     &45000          &\textgreater45000 &50000          &840           &\textgreater55000 &\textgreater55000 &\textgreater55000\\\hline
% \end{tabular}

==> tables/shifts.tex <==
% \toprule
\begin{table*}[ht]
\centering
\small
\begin{tabular}{ | c | c | c | c |}
  \midrule  \textbf{Dataset} & Shift Type & Source Set & Target Set \\ \midrule
Camelyon17 & shift & $split\in\{0, 1\}$ & $split\in\{2, 3, 4\}$ \\ 
\midrule 
iWildCam & shift & $split\in\{val,$ $test\}$ & $split\in\{id\_val,$  $id\_test,$ $train\}$ \\ 
\midrule 
FMoW & shift & $split=train$ & $split\neq train$ \\ 
\midrule
CIFAR10 & shift & $split=\text{low average pixel value}$ & $split=\text{high average pixel value}$ \\ 
\midrule
CIFAR100 & shift & $split=\text{low average pixel value}$ & $split=\text{high average pixel value}$ \\ 
\midrule
SVHN & shift & $split=\text{low average pixel value}$ & $split=\text{high average pixel value}$ \\ 
\midrule
MNIST & shift & $split=\text{low average pixel value}$ & $split=\text{high average pixel value}$ \\ 
\midrule 
\end{tabular}
\caption{\label{tab:shifts-table} A description of how the source and target datasets are created in the shift settings.}
\end{table*} 
